StepMix: A Python Package for Pseudo-Likelihood Estimation of Generalized Mixture Models with External Variables

StepMix is an open-source Python package for the pseudo-likelihood estimation (one-, two- and three-step approaches) of generalized finite mixture models (latent profile and latent class analysis) with external variables (covariates and distal outcomes). In many applications in social sciences, the main objective is not only to cluster individuals into latent classes, but also to use these classes to develop more complex statistical models. These models generally divide into a measurement model that relates the latent classes to observed indicators, and a structural model that relates covariates and outcome variables to the latent classes. The measurement and structural models can be estimated jointly using the so-called one-step approach or sequentially using stepwise methods, which present significant advantages for practitioners regarding the interpretability of the estimated latent classes. In addition to the one-step approach, StepMix implements the most important stepwise estimation methods from the literature, including the bias-adjusted three-step methods with Bolk-Croon-Hagenaars and maximum likelihood corrections and the more recent two-step approach. These pseudo-likelihood estimators are presented in this paper under a unified framework as specific expectation-maximization subroutines. To facilitate and promote their adoption among the data science community, StepMix follows the object-oriented design of the scikit-learn library and provides an additional R wrapper.

==> pseudocode/old_3_step_bch.tex <==
\begin{algorithm}[H]
\caption{BCH three-step method}\label{alg:3-step-bch}
\begin{algorithmic}

%Initialization
\State Initialize $\hat{\theta}_M^{(0)}=(\hat{\theta}_X^{(0)},  \hat{\theta}_Y^{(0)})$ \\
\vspace{-0.2cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 1 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrulefill
\State \underline{\textbf{STEP 1 : EM algorithm on the MM}}

%Iteration counter
\State Set $t=0$

%EM iterations
\Repeat
\vspace{-0.1cm}

    %E Step
    \State \hrulefill \text{ E Step }\hrulefill
    
    %Update responsibilities
    \State $\tau^{(t)}_{ik} = p(X_i{=}k|y_i;\hat{\theta}_M^{(t)}), \ \forall i \in N_1, \forall k \in \mathcal{X}$ \Comment{Update responsibilities}
    \vspace{0.2cm}

    %M Step
    \State \hrulefill \text{ M Step }\hrulefill

    %Update \theta_X
    \State $\hat{\theta}_{X}^{(t+1)} = \argmax\limits_{\theta_{X} \in \Theta_{X}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(X_i{=}k;\theta_{X})$
    \Comment{Update $\hat{\theta}_{X}$}

    %Update \theta_Y
    \State $\hat{\theta}_{Y}^{(t+1)} = \argmax\limits_{\theta_{Y} \in \Theta_{Y}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(y_i|X_i{=}k;\theta_{Y})$
    \Comment{Update $\hat{\theta}_{Y}$}

    %Iteration counter
    \State $t=t+1$
\Until{convergence}

%Two-step SM parameters estimators
\State Set $\hat{\theta}_M = (\hat{\theta}_X^{(t)},\hat{\theta}_Y^{(t)})$ \Comment{Estimated MM parameters}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 2 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 2 : Bias-adjusted class weights based on the MM}}

%Predicted class membership
\State Set $\tilde{x}_j = \argmax_{k \in \mathcal{X}}p(X_j{=}k|y_j;\hat{\theta}_M), \ \forall j \in N_2$\Comment{Predicted class membership}

%Soft or modal weights
\State Set $w_{jk}=\begin{cases}
    p(X_j{=}k|y_j;\hat{\theta}_M) & \text{, if soft assignments}\\
    \mathds{1}[\tilde{x}_j{=}k] & \text{, if modal assignments}
\end{cases}, \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Unadjusted weights}

%Estimated misclassification probabilities
\State Set $D_{ck} = p(\tilde{X}_j{=}k|X_j{=}c; \hat{\theta}_M), \ \forall (c,k) \in \mathcal{X}^2$  \Comment{Estimated misclassification probabilities}

%Bias-adjusted weights
\State Set $w^*_{j} = w_j D^{-1}$ \hspace{0.5cm} $\forall j \in N_2$  \Comment{Bias-adjusted weights}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 3 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 3 : MPLE of the SM parameters based on imputed class weights}}

%Estimate \theta_{Z^p}
\State $\hat{\theta}_{Z^p} = \argmax\limits_{\theta_{Z^p} \in \Theta_{Z^p}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w^*_{jk}\log p(X_j{=}k;z^p_j,\theta_{Z^p})$
\Comment{Compute $\hat{\theta}_{Z^p}$}

%Estimate \theta_{Z^o}
\State $\hat{\theta}_{Z^o} = \argmax\limits_{\theta_{Z^o} \in \Theta_{Z^o}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w^*_{jk}\log p(z^o_j|X_j{=}k;\theta_{Z^o})$
\Comment{Compute $\hat{\theta}_{Z^o}$}

%Three-step SM parameters estimators
\State Set $\hat{\theta}_S = (\hat{\theta}_{Z^p}, \hat{\theta}_{Z^o})$ \Comment{Estimated SM parameters}

%Return
\\\hrulefill
\State Return $(\hat{\theta}_M, \hat{\theta}_S)$ \Comment{Estimated CM parameters}
\end{algorithmic}
\end{algorithm}

==> pseudocode/old_3_step_ml.tex <==
\begin{algorithm}[H]
\caption{ML three-step method}\label{alg:3-step-ml}
\begin{algorithmic}

%Initialization
\State Initialize $\hat{\theta}_M^{(0)}=(\hat{\theta}_X^{(0)},  \hat{\theta}_Y^{(0)})$ and $\hat{\theta}_S^{(0)}=(\hat{\theta}_{Z^o}^{(0)},  \hat{\theta}_{Z^p}^{(0)})$\\
\vspace{-0.2cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 1 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrulefill
\State \underline{\textbf{STEP 1 : EM algorithm on the MM}}

%Iteration counter
\State Set $t=0$

%EM iterations
\Repeat
\vspace{-0.1cm}

    %E Step
    \State \hrulefill \text{ E Step }\hrulefill
    
    %Update responsibilities
    \State $\tau^{(t)}_{ik} = p(X_i{=}k|y_i;\hat{\theta}_M^{(t)}), \ \forall i \in N_1, \forall k \in \mathcal{X}$ \Comment{Update responsibilities}
    \vspace{0.2cm}

    %M Step
    \State \hrulefill \text{ M Step }\hrulefill

    %Update \theta_X
    \State $\hat{\theta}_{X}^{(t+1)} = \argmax\limits_{\theta_{X} \in \Theta_{X}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(X_i{=}k;\theta_{X})$
    \Comment{Update $\hat{\theta}_{X}$}

    %Update \theta_Y
    \State $\hat{\theta}_{Y}^{(t+1)} = \argmax\limits_{\theta_{Y} \in \Theta_{Y}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(y_i|X_i{=}k;\theta_{Y})$
    \Comment{Update $\hat{\theta}_{Y}$}

    %Iteration counter
    \State $t=t+1$
\Until{convergence}

%Two-step SM parameters estimators
\State Set $\hat{\theta}_M = (\hat{\theta}_X^{(t)},\hat{\theta}_Y^{(t)})$ \Comment{Estimated MM parameters}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 2 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 2 : Class weights and misclassification probabilities based on the MM}}

%Predicted class membership
\State Set $\tilde{x}_j = \argmax_{k \in \mathcal{X}}p(X_j{=}k|y_j;\hat{\theta}_M), \ \forall j \in N_2$\Comment{Predicted class membership}

%Soft or modal weights
\State Set $w_{jk}=\begin{cases}
    p(X_j{=}k|y_j;\hat{\theta}_M) & \text{, if soft assignments}\\
    \mathds{1}[\tilde{x}_j{=}k] & \text{, if modal assignments}
\end{cases}, \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Weights}

%Estimated misclassification probabilities
\State Set $D_{ck} = p(\tilde{X}_j{=}k|X_j{=}c; \hat{\theta}_M), \ \forall (c,k) \in \mathcal{X}^2$  \Comment{Estimated misclassification probabilities}

%Estimated class membership probabilities
\State $w=wD^{T}$  \Comment{Estimated class membership probabilities}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 3 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 3 : EM algorithm on the SM, augmented with predicted class memberships}}

%Iteration counter
\State Set $t=0$

%EM iterations
\Repeat
\vspace{-0.1cm}

    %E Step
    \State \hrulefill \text{ E Step }\hrulefill
    
    %Update responsibilities
    \State $\tau^{(t)}_{jk} = w_{jk}p(X_j{=}k|z^o_j;z^p_j,\hat{\theta}_S^{(t)}), \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Update responsibilities}
    \State $\tau^{(t)}_{jk} = \frac{\tau^{(t)}_{jk}}{\sum_{c \in \mathcal{X}}\tau^{(t)}_{jc}} \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Normalize responsibilities}
    \vspace{0.2cm}

    %M Step
    \State \hrulefill \text{ M Step }\hrulefill

    %Update \theta_{Z^p}
    \State $\hat{\theta}_{Z^p}^{(t+1)} = \argmax\limits_{\theta_{Z^p} \in \Theta_{Z^p}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{jk}\log p(X_j{=}k;z^p_j,\theta_{Z^p})$
    \Comment{Update $\hat{\theta}_{Z^p}$}

    %Update \theta_{Z^o}
    \State $\hat{\theta}_{Z^o}^{(t+1)} = \argmax\limits_{\theta_{Z^o} \in \Theta_{Z^o}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{jk}\log p(z^o_j|X_j{=}k;\theta_{Z^o})$
    \Comment{Update $\hat{\theta}_{Z^o}$}

    %Iteration counter
    \State $t=t+1$
\Until{convergence}

%Two-step SM parameters estimators
\State Set $\hat{\theta}_S = (\hat{\theta}_{Z^p}^{(t)}, \hat{\theta}_{Z^o}^{(t)})$ \Comment{Estimated SM parameters}

%Return
\\\hrulefill
\State Return $(\hat{\theta}_M, \hat{\theta}_S)$ \Comment{Estimated CM parameters}
\end{algorithmic}
\end{algorithm}

==> pseudocode/old_3_step_naive.tex <==
\begin{algorithm}[H]
\caption{Naive three-step method}\label{alg:3-step-naive}
\begin{algorithmic}

%Initialization
\State Initialize $\hat{\theta}_M^{(0)}=(\hat{\theta}_X^{(0)},  \hat{\theta}_Y^{(0)})$\\
\vspace{-0.2cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 1 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrulefill
\State \underline{\textbf{STEP 1 : EM algorithm on the MM}}

%Iteration counter
\State Set $t=0$

%EM iterations
\Repeat
\vspace{-0.1cm}

    %E Step
    \State \hrulefill \text{ E Step }\hrulefill
    
    %Update responsibilities
    \State $\tau^{(t)}_{ik} = p(X_i{=}k|y_i;\hat{\theta}_M^{(t)}), \ \forall i \in N_1, \forall k \in \mathcal{X}$ \Comment{Update responsibilities}
    \vspace{0.2cm}

    %M Step
    \State \hrulefill \text{ M Step }\hrulefill

    %Update \theta_X
    \State $\hat{\theta}_{X}^{(t+1)} = \argmax\limits_{\theta_{X} \in \Theta_{X}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(X_i{=}k;\theta_{X})$
    \Comment{Update $\hat{\theta}_{X}$}

    %Update \theta_Y
    \State $\hat{\theta}_{Y}^{(t+1)} = \argmax\limits_{\theta_{Y} \in \Theta_{Y}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(y_i|X_i{=}k;\theta_{Y})$
    \Comment{Update $\hat{\theta}_{Y}$}

    %Iteration counter
    \State $t=t+1$
\Until{convergence}

%Two-step SM parameters estimators
\State Set $\hat{\theta}_M = (\hat{\theta}_X^{(t)},\hat{\theta}_Y^{(t)})$ \Comment{Estimated MM parameters}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 2 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 2 : Class weights based on the MM}}

%Predicted class membership
\State Set $\tilde{x}_j = \argmax_{k \in \mathcal{X}}p(X_j{=}k|y_j;\hat{\theta}_M), \ \forall j \in N_2$\Comment{Predicted class membership}

%Soft or modal weights
\State Set $w_{jk}=\begin{cases}
    p(X_j{=}k|y_j;\hat{\theta}_M) & \text{, if soft assignments}\\
    \mathds{1}[\tilde{x}_j{=}k] & \text{, if modal assignments}
\end{cases}, \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Weights}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 3 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 3 : MPLE of the SM parameters based on imputed class weights}}

%Estimate \theta_{Z^p}
\State $\hat{\theta}_{Z^p} = \argmax\limits_{\theta_{Z^p} \in \Theta_{Z^p}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w_{jk}\log p(X_j{=}k;z^p_j,\theta_{Z^p})$
\Comment{Compute $\hat{\theta}_{Z^p}$}

%Estimate \theta_{Z^o}
\State $\hat{\theta}_{Z^o} = \argmax\limits_{\theta_{Z^o} \in \Theta_{Z^o}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w_{jk}\log p(z^o_j|X_j{=}k;\theta_{Z^o})$
\Comment{Compute $\hat{\theta}_{Z^o}$}

%Three-step SM parameters estimators
\State Set $\hat{\theta}_S = (\hat{\theta}_{Z^p}, \hat{\theta}_{Z^o})$ \Comment{Estimated SM parameters}

%Return
\\\hrulefill
\State Return $(\hat{\theta}_M, \hat{\theta}_S)$ \Comment{Estimated CM parameters}
\end{algorithmic}
\end{algorithm}

==> pseudocode/old_3_step_naive_bch.tex <==
\begin{algorithm}[H]
\caption{Naive or BCH three-step method}\label{alg:3-step-naive}
\begin{algorithmic}

%Initialization
\State Initialize $\hat{\theta}_M^{(0)}=(\hat{\theta}_X^{(0)},  \hat{\theta}_Y^{(0)})$\\
\vspace{-0.2cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 1 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrulefill
\State \underline{\textbf{STEP 1 : EM algorithm on the MM}}

%Iteration counter
\State Set $t=0$

%EM iterations
\Repeat
\vspace{-0.1cm}

    %E Step
    \State \hrulefill \text{ E Step }\hrulefill
    
    %Update responsibilities
    \State $\tau^{(t)}_{ik} = p(X_i{=}k|y_i;\hat{\theta}_M^{(t)}), \ \forall i \in N_1, \forall k \in \mathcal{X}$ \Comment{Update responsibilities}
    \vspace{0.2cm}

    %M Step
    \State \hrulefill \text{ M Step }\hrulefill

    %Update \theta_X
    \State $\hat{\theta}_{X}^{(t+1)} = \argmax\limits_{\theta_{X} \in \Theta_{X}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(X_i{=}k;\theta_{X})$
    \Comment{Update $\hat{\theta}_{X}$}

    %Update \theta_Y
    \State $\hat{\theta}_{Y}^{(t+1)} = \argmax\limits_{\theta_{Y} \in \Theta_{Y}}\sum\limits_{i\in N_1}\omega_i\sum\limits_{k\in\mathcal{X}} \tau^{(t)}_{ik}\log p(y_i|X_i{=}k;\theta_{Y})$
    \Comment{Update $\hat{\theta}_{Y}$}

    %Iteration counter
    \State $t=t+1$
\Until{convergence}

%Two-step SM parameters estimators
\State Set $\hat{\theta}_M = (\hat{\theta}_X^{(t)},\hat{\theta}_Y^{(t)})$ \Comment{Estimated MM parameters}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 2 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 2 : Class weights based on the MM}}

%Predicted class membership
\State Set $\tilde{x}_j = \argmax_{k \in \mathcal{X}}p(X_j{=}k|y_j;\hat{\theta}_M), \ \forall j \in N_2$\Comment{Predicted class membership}

%Soft or modal weights
\State Set $w_{jk}=\begin{cases}
    p(X_j{=}k|y_j;\hat{\theta}_M) & \text{, if soft assignments}\\
    \mathds{1}[\tilde{x}_j{=}k] & \text{, if modal assignments}
\end{cases}, \ \forall j \in N_2, \forall k \in \mathcal{X}$ \Comment{Unadjusted weights}

\If{BCH}
%Estimated misclassification probabilities
\State Set $D_{ck} = p(\tilde{X}_j{=}k|X_j{=}c; \hat{\theta}_M), \ \forall (c,k) \in \mathcal{X}^2$  \Comment{Estimated misclassification probabilities}

%Bias-adjusted weights
\State $w = wD^{-1}$  \Comment{Bias-adjusted weights}
\EndIf

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STEP 3 of 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\\hrulefill
\State \underline{\textbf{STEP 3 : MPLE of the SM parameters based on imputed class weights}}

%Estimate \theta_{Z^p}
\State $\hat{\theta}_{Z^p} = \argmax\limits_{\theta_{Z^p} \in \Theta_{Z^p}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w_{jk}\log p(X_j{=}k;z^p_j,\theta_{Z^p})$
\Comment{Compute $\hat{\theta}_{Z^p}$}

%Estimate \theta_{Z^o}
\State $\hat{\theta}_{Z^o} = \argmax\limits_{\theta_{Z^o} \in \Theta_{Z^o}}\sum\limits_{j\in N_2}\omega_j\sum\limits_{k\in\mathcal{X}} w_{jk}\log p(z^o_j|X_j{=}k;\theta_{Z^o})$
\Comment{Compute $\hat{\theta}_{Z^o}$}

%Three-step SM parameters estimators
\State Set $\hat{\theta}_S = (\hat{\theta}_{Z^p}, \hat{\theta}_{Z^o})$ \Comment{Estimated SM parameters}

%Return
\\\hrulefill
\State Return $(\hat{\theta}_M, \hat{\theta}_S)$ \Comment{Estimated CM parameters}
\end{algorithmic}
\end{algorithm}
